Do A-type stars flare?

For flares to be generated, stars have to have a sufficiently deep outer convection zone (F5 and later), strong large--scale magnetic fields (Ap/Bp-type stars) or strong, radiatively driven winds (B5 and earlier). Normal A-type stars possess none of these and therefore should not flare. Nevertheless, flares have previously been detected in the Kepler lightcurves of 33 A-type stars and interpreted to be intrinsic to the stars. Here we present new and detailed analyses of these 33 stars, imposing very strict criteria for the flare detection. We confirm the presence of flare-like features in 27 of the 33 A-type stars. A study of the pixel data and the surrounding field-of-view (FOV) reveals that 14 of these 27 flaring objects have overlapping neighbouring stars and 5 stars show clear contamination in the pixel data. We have obtained high-resolution spectra for 2/3 of the entire sample and confirm that our targets are indeed A-type stars. Detailed analyses revealed that 11 out of 19 stars with multiple epochs of observations are spectroscopic binaries. Furthermore, and contrary to previous studies, we find that the flares can originate from a cooler, unresolved companion. We note the presence of H$\alpha$ emission in eight stars. Whether this emission is circumstellar or magnetic in origin is unknown. In summary, we find possible alternative explanations for the observed flares for at least 19 of the 33 A-type stars, but find no truly convincing target to support the hypothesis of flaring A-type stars.

==> references <==
@BOOK{Allen1973,
   author = {{Allen}, C.~W.},
    title = "{Astrophysical quantities}",
 keywords = {ASTROPHYSICS, ASTRONOMICAL CONSTANTS, TABLES, HANDBOOKS},
booktitle = {London: University of London, Athlone Press, |c1973, 3rd ed.},
     year = 1973,
   adsurl = {http://adsabs.harvard.edu/abs/1973asqu.book.....A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  place = {London},
  publisher = {University of London, Athlone Press},
  edition = third
}

@ARTICLE{Balona2012,
   author = {{Balona}, L.~A.},
    title = "{Kepler observations of flaring in A-F type stars}",
  journal = {\mnras},
 keywords = {stars: activity, stars: flare, starspots},
     year = 2012,
    month = jul,
   volume = 423,
    pages = {3420-3429},
      doi = {10.1111/j.1365-2966.2012.21135.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.423.3420B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Balona2013,
   author = {{Balona}, L.~A.},
    title = "{Activity in A-type stars}",
  journal = {\mnras},
 keywords = {stars: activity, stars: oscillations, stars: rotation, starspots, stars: variables: general},
     year = 2013,
    month = may,
   volume = 431,
    pages = {2240-2252},
      doi = {10.1093/mnras/stt322},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.431.2240B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Balona2015,
   author = {{Balona}, L.~A.},
    title = "{Flare stars across the H-R diagram}",
  journal = {IAU General Assembly},
     year = 2015,
    month = aug,
   volume = 22,
      eid = {2242630},
    pages = {2242630},
   adsurl = {http://adsabs.harvard.edu/abs/2015IAUGA..2242630B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Batalha2010,
   author = {{Batalha}, N.~M. and {Borucki}, W.~J. and {Koch}, D.~G. and 
	{Bryson}, S.~T. and {Haas}, M.~R. and {Brown}, T.~M. and {Caldwell}, D.~A. and 
	{Hall}, J.~R. and {Gilliland}, R.~L. and {Latham}, D.~W. and 
	{Meibom}, S. and {Monet}, D.~G.},
    title = "{Selection, Prioritization, and Characteristics of Kepler Target Stars}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1001.0349},
 primaryClass = "astro-ph.SR",
 keywords = {planetary systems, stars: statistics},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {L109-L114},
      doi = {10.1088/2041-8205/713/2/L109},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713L.109B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bertaux2014,
   author = {{Bertaux}, J.~L. and {Lallement}, R. and {Ferron}, S. and {Boonne}, C. and 
	{Bodichon}, R.},
    title = "{TAPAS, a web-based service of atmospheric transmission computation for astronomy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1311.4169},
 primaryClass = "astro-ph.IM",
 keywords = {atmospheric effects, techniques: spectroscopic},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A46},
    pages = {A46},
      doi = {10.1051/0004-6361/201322383},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..46B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Bertaux2014b,
   author = {{Bertaux}, J.-L. and {Lallement}, R. and {Ferron}, S. and {Boonne}, C.
	},
    title = "{TAPAS, a web-based service of atmospheric transmission computation for astronomy}",
booktitle = {13th International HITRAN Conference},
     year = 2014,
    month = jun,
      doi = {10.5281/zenodo.11110},
   adsurl = {http://adsabs.harvard.edu/abs/2014hitr.confE...8B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Boch2014,
   author = {{Boch}, T. and {Fernique}, P.},
    title = "{Aladin Lite: Embed your Sky in the Browser}",
booktitle = {Astronomical Data Analysis Software and Systems XXIII},
     year = 2014,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 485,
   editor = {{Manset}, N. and {Forshay}, P.},
    month = may,
    pages = {277},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014ASPC..485..277B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonnarel2000,
   author = {{Bonnarel}, F. and {Fernique}, P. and {Bienaym{\'e}}, O. and 
	{Egret}, D. and {Genova}, F. and {Louys}, M. and {Ochsenbein}, F. and 
	{Wenger}, M. and {Bartlett}, J.~G.},
    title = "{The ALADIN interactive sky atlas. A reference tool for identification of astronomical sources}",
  journal = {\aaps},
 keywords = {ASTRONOMICAL DATA BASES: MISCELLANEOUS, CATALOGS, ATLASES, SURVEYS},
     year = 2000,
    month = apr,
   volume = 143,
    pages = {33-40},
      doi = {10.1051/aas:2000331},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2000A%26AS..143...33B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Braithwaite2014,
   author = {{Braithwaite}, J.},
    title = "{The nature and origin of magnetic fields in early-type stars}",
 keywords = {stars: activity, stars: magnetic fields, stars: early-type, stars: chemically peculiar,},
booktitle = {Magnetic Fields throughout Stellar Evolution},
     year = 2014,
   series = {IAU Symposium},
   volume = 302,
archivePrefix = "arXiv",
   eprint = {1312.4755},
 primaryClass = "astro-ph.SR",
   editor = {{Petit}, P. and {Jardine}, M. and {Spruit}, H.~C.},
    month = aug,
    pages = {255-264},
      doi = {10.1017/S1743921314002221},
   adsurl = {http://adsabs.harvard.edu/abs/2014IAUS..302..255B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Briquet2010,
   author = {{Briquet}, M. and {Korhonen}, H. and {Gonz{\'a}lez}, J.~F. and 
	{Hubrig}, S. and {Hackman}, T.},
    title = "{Dynamical evolution of titanium, strontium, and yttrium spots on the surface of the HgMn star <ASTROBJ>HD 11753</ASTROBJ>}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1003.1902},
 primaryClass = "astro-ph.SR",
 keywords = {stars: chemically peculiar, stars: individual: HD 11753, stars: individual: HD 53244, stars: individual: HD 221507, stars: variables: general},
     year = 2010,
    month = feb,
   volume = 511,
      eid = {A71},
    pages = {A71},
      doi = {10.1051/0004-6361/200913775},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...511A..71B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brown2011,
   author = {{Brown}, T.~M. and {Latham}, D.~W. and {Everett}, M.~E. and 
	{Esquerdo}, G.~A.},
    title = "{Kepler Input Catalog: Photometric Calibration and Stellar Classification}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1102.0342},
 primaryClass = "astro-ph.SR",
 keywords = {catalogs, methods: data analysis, surveys, techniques: photometric},
     year = 2011,
    month = oct,
   volume = 142,
      eid = {112},
    pages = {112},
      doi = {10.1088/0004-6256/142/4/112},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....142..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brun2005,
   author = {{Brun}, A.~S. and {Browning}, M.~K. and {Toomre}, J.},
    title = "{Simulations of Core Convection in Rotating A-Type Stars: Magnetic Dynamo Action}",
  journal = {\apj},
   eprint = {astro-ph/0610072},
 keywords = {Convection, Magnetohydrodynamics: MHD, Stars: Evolution, Stars: Interiors, Stars: Magnetic Fields},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {461-481},
      doi = {10.1086/430430},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..461B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Bryson2010a,
   author = {{Bryson}, S.~T. and {Jenkins}, J.~M. and {Klaus}, T.~C. and 
	{Cote}, M.~T. and {Quintana}, E.~V. and {Hall}, J.~R. and {Ibrahim}, K. and 
	{Chandrasekaran}, H. and {Caldwell}, D.~A. and {Van Cleve}, J.~E. and 
	{Haas}, M.~R.},
    title = "{Selecting pixels for Kepler downlink}",
booktitle = {Software and Cyberinfrastructure for Astronomy},
     year = 2010,
   series = {\procspie},
   volume = 7740,
    month = jul,
      eid = {77401D},
    pages = {77401D},
      doi = {10.1117/12.857625},
   adsurl = {http://adsabs.harvard.edu/abs/2010SPIE.7740E..1DB},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cardelli1986,
   author = {{Cardelli}, J.~A. and {Wallerstein}, G.},
    title = "{Visual absorption lines in dark clouds - Highly reddened stars near the center of the Ophiuchus molecular cloud}",
  journal = {\apj},
 keywords = {Absorption Spectra, Interstellar Chemistry, Interstellar Extinction, Molecular Clouds, Ophiuchi Clouds, Stellar Spectra, Abundance, Cn Emission, Electron Density (Concentration), Molecular Spectra, Nebulae, Radial Velocity, Visible Spectrum},
     year = 1986,
    month = mar,
   volume = 302,
    pages = {492-503},
      doi = {10.1086/164008},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...302..492C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Catanzaro2014,
   author = {{Catanzaro}, G. and {Ripepi}, V.},
    title = "{Fundamental parameters of eight Am stars: comparing observations with theory}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.0954},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: chemically peculiar, stars: early-type, stars: fundamental parameters},
     year = 2014,
    month = jun,
   volume = 441,
    pages = {1669-1680},
      doi = {10.1093/mnras/stu674},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014MNRAS.441.1669C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Capelli2011,
   author = {{Capelli}, R. and {Warwick}, R.~S. and {Cappelluti}, N. and 
	{Gillessen}, S. and {Predehl}, P. and {Porquet}, D. and {Czesla}, S.
	},
    title = "{Discovery of X-ray flaring activity in the Arches cluster}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1011.4062},
 primaryClass = "astro-ph.HE",
 keywords = {stars: flare, galaxy: center, X-rays: stars},
     year = 2011,
    month = jan,
   volume = 525,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201015758},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...525L...2C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carrington1859,
   author = {{Carrington}, R.~C.},
    title = "{Description of a Singular Appearance seen in the Sun on September 1, 1859}",
  journal = {\mnras},
     year = 1859,
    month = nov,
   volume = 20,
    pages = {13-15},
      doi = {10.1093/mnras/20.1.13},
   adsurl = {http://adsabs.harvard.edu/abs/1859MNRAS..20...13C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Castelli2004,
   author = {{Castelli}, F. and {Kurucz}, R.~L.},
    title = "{New Grids of ATLAS9 Model Atmospheres}",
  journal = {ArXiv Astrophysics e-prints},
   eprint = {astro-ph/0405087},
 keywords = {Astrophysics},
     year = 2004,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2004astro.ph..5087C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Charbonneau2010,
   author = {{Charbonneau}, P.},
    title = "{Dynamo Models of the Solar Cycle}",
  journal = {Living Rev. Solar Phys.},
     year = 2010,
   volume = 7,
    pages = 3,
   adsurl = {http://www.livingreviews.org/lrsp-2010-3}
}

@ARTICLE{Chabrier1997,
   author = {{Chabrier}, G. and {Baraffe}, I.},
    title = "{Structure and evolution of low-mass stars}",
  journal = {\aap},
   eprint = {astro-ph/9704118},
 keywords = {STARS: LOW MASS, BROWN DWARFS, STARS: ABUNDANCES},
     year = 1997,
    month = nov,
   volume = 327,
    pages = {1039-1053},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...327.1039C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Coughlin2014,
   author = {{Coughlin}, J.~L. and {Thompson}, S.~E. and {Bryson}, S.~T. and 
	{Burke}, C.~J. and {Caldwell}, D.~A. and {Christiansen}, J.~L. and 
	{Haas}, M.~R. and {Howell}, S.~B. and {Jenkins}, J.~M. and {Kolodziejczak}, J.~J. and 
	{Mullally}, F.~R. and {Rowe}, J.~F.},
    title = "{Contamination in the Kepler Field. Identification of 685 KOIs as False Positives via Ephemeris Matching Based on Q1-Q12 Data}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1401.1240},
 primaryClass = "astro-ph.IM",
 keywords = {binaries: eclipsing, instrumentation: detectors, planetary systems, planets and satellites: detection, stars: statistics, techniques: photometric},
     year = 2014,
    month = may,
   volume = 147,
      eid = {119},
    pages = {119},
      doi = {10.1088/0004-6256/147/5/119},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....147..119C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cowling1945,
   author = {{Cowling}, T.~G.},
    title = "{On the Sun's general magnetic field}",
  journal = {\mnras},
     year = 1945,
   volume = 105,
    pages = {166},
      doi = {10.1093/mnras/105.3.166},
   adsurl = {http://adsabs.harvard.edu/abs/1945MNRAS.105..166C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chabrier2006,
   author = {{Chabrier}, G. and {K{\"u}ker}, M.},
    title = "{Large-scale {$\alpha$}\^{}2-dynamo in low-mass stars and brown dwarfs}",
  journal = {\aap},
   eprint = {astro-ph/0510075},
 keywords = {magnetohydrodynamics (MHD), turbulence, stars: activity, stars: chromosphere, stars: low mass, brown dwarfs},
     year = 2006,
    month = feb,
   volume = 446,
    pages = {1027-1037},
      doi = {10.1051/0004-6361:20042475},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...446.1027C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{ChristiansenVanCleve2011,
   author = {{Christiansen}, J.~L. and {Jenkins}, J.~M. and {Caldwell}, D.~A. and {Barclay}, T. and {Bryson}, S.~T. and {Burke}, C.~J. and {Campbell}, J. and {Catanzarite}, J. and {Clarke}, B.~D. and {Coughlin}, J.~L. and {Girouard}, F. and {Haas}, M.~R. and {Ibrahim}, K. and {Klaus}, T.~C. and {Kolodziejczak}, J.~J. and {Li}, J. and {McCauliff}, S.~D. and {Morris}, R.~L. and {Mullally}, F. and {Quintana}, E.~V. and {Rowe}, J. and {Sabale}, A. and {Seader}, S. and {Smith}, J.~C. and {Still}, M.~D. and {Tenenbaum}, P.~G. and {Thompson}, S.~E. and {Twicken}, J.~D. and {Uddin}, A.~K.},
    title = "{Kepler Data Characteristics Handbook, KSCI 19040-004}",
booktitle = {Kepler Data Characteristics Handbook},
     year = 2013,
   adsurl = {https://archive.stsci.edu/kepler/manuals/Data_Characteristics.pdf},
  Publisher = {NASA Ames Research Center},
  place = {Moffett Field, CA. 94035}
}

 

@ARTICLE{Donati2002,
   author = {{Donati}, J.-F. and {Babel}, J. and {Harries}, T.~J. and {Howarth}, I.~D. and 
	{Petit}, P. and {Semel}, M.},
    title = "{The magnetic field and wind confinement of {\thetas}$^{1}$ Orionis C}",
  journal = {\mnras},
 keywords = {stars: individual: {\thetas}1 Ori C, stars: magnetic fields, stars: rotation, stars: winds, outflows},
     year = 2002,
    month = jun,
   volume = 333,
    pages = {55-70},
      doi = {10.1046/j.1365-8711.2002.05379.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.333...55D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dudorov2015,
   author = {{Dudorov}, A.~E. and {Khaibrakhmanov}, S.~A.},
    title = "{Theory of fossil magnetic field}",
  journal = {Advances in Space Research},
archivePrefix = "arXiv",
   eprint = {1406.4663},
 primaryClass = "astro-ph.SR",
 keywords = {Young stars, Accretion disks, Magnetic fields, Diffusion},
     year = 2015,
    month = feb,
   volume = 55,
    pages = {843-850},
      doi = {10.1016/j.asr.2014.05.034},
   adsurl = {http://adsabs.harvard.edu/abs/2015AdSpR..55..843D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Duflot1995,
   author = {{Duflot}, M. and {Figon}, P. and {Meyssonnier}, N.},
    title = "{Vitesses radiales. Catalogue WEB: Wilson Evans Batten. Subtittle: Radial velocities: The Wilson-Evans-Batten catalogue.}",
  journal = {\aaps},
 keywords = {RADIAL VELOCITIES, CATALOGUES, STARS: KINEMATIC},
     year = 1995,
    month = dec,
   volume = 114,
    pages = {269},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1995A%26AS..114..269D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Durney1993,
   author = {{Durney}, B.~R. and {De Young}, D.~S. and {Roxburgh}, I.~W.},
    title = "{On the generation of the large-scale and turbulent magnetic fields in solar-type stars}",
  journal = {\solphys},
 keywords = {Dynamo Theory, Magnetohydrodynamic Turbulence, Solar Convection (Astronomy), Solar Magnetic Field, Stellar Interiors, Chromosphere, Helices, Poloidal Flux, Solar Radiation, Stellar Rotation},
     year = 1993,
    month = jun,
   volume = 145,
    pages = {207-225},
      doi = {10.1007/BF00690652},
   adsurl = {http://adsabs.harvard.edu/abs/1993SoPh..145..207D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fehrenbach1990,
   author = {{Fehrenbach}, C. and {Burnage}, R.},
    title = "{Radial-velocity measurements. III - Ground observations accompanying the HIPPARCOS satellite observation program: Measurements of the radial velocities of 391 stars in 12 fields}",
  journal = {\aaps},
 keywords = {Radial Velocity, Sky Surveys (Astronomy), Astronomical Catalogs, Celestial Mechanics, Hipparcos Satellite},
     year = 1990,
    month = apr,
   volume = 83,
    pages = {91-107},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1990A%26AS...83...91F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fehrenbach1997,
   author = {{Fehrenbach}, C. and {Duflot}, M. and {Mannone}, C. and {Burnage}, R. and 
	{Genty}, V.},
    title = "{Mesures de vitesses radiales. VIII. Accompagnement AU sol du programme d'observation du satellite HIPPARCOS}",
  journal = {\aaps},
 keywords = {TECHNIQUES: RADIAL VELOCITIES, CATALOGUES, GALAXY: KINEMATICS AND DYNAMICS},
     year = 1997,
    month = aug,
   volume = 124,
    pages = {255-257},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26AS..124..255F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Floquet1975,
   author = {{Floquet}, M.},
    title = "{Spectral classification of Ap and Am stars.}",
  journal = {\aaps},
     year = 1975,
    month = jul,
   volume = 21,
    pages = {25-32},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1975A%26AS...21...25F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Gagne2016,
       author = {{Gagne}, M. and {Owocki}, S. and {Sundqvist}, J. and {ud-Doula}, A.},
       title = "{Private communication}",
       year = "2016" }

@ARTICLE{Gizis2002,
   author = {{Gizis}, J.~E. and {Reid}, I.~N. and {Hawley}, S.~L.},
    title = "{The Palomar/MSU Nearby Star Spectroscopic Survey. III. Chromospheric Activity, M Dwarf Ages, and the Local Star Formation History}",
  journal = {\aj},
   eprint = {astro-ph/0203499},
 keywords = {Galaxy: Formation, Galaxy: Solar Neighborhood, Stars: Chromospheres, Stars: Formation, Stars: Low-Mass, Brown Dwarfs},
     year = 2002,
    month = jun,
   volume = 123,
    pages = {3356-3369},
      doi = {10.1086/340465},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....123.3356G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gontcharov2006,
   author = {{Gontcharov}, G.~A.},
    title = "{Pulkovo Compilation of Radial Velocities for 35 495 Hipparcos stars in a common system}",
  journal = {Astronomy Letters},
     year = 2006,
    month = nov,
   volume = 32,
    pages = {759-771},
      doi = {10.1134/S1063773706110065},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006AstL...32..759G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{GrayAtmosphere,
	author = {{Gray}, David F.},
	title = {The Observation and Analysis of Stellar Photospheres},
	publisher = {Cambridge University Press},
	place = {New York},
	year = {2008},
	edition = {Third}
}

@ARTICLE{Gray1994,
   author = {{Gray}, R.~O. and {Corbally}, C.~J.},
    title = "{The calibration of MK spectral classes using spectral synthesis. 1: The effective temperature calibration of dwarf stars}",
  journal = {\aj},
 keywords = {Atmospheric Models, Calibrating, Classifications, Dwarf Stars, Standards, Stellar Atmospheres, Stellar Models, Stellar Spectra, Stellar Temperature, Visible Spectrum, Applications Programs (Computers), Astronomical Spectroscopy, Charge Coupled Devices, Ibm Personal Computers, Light (Visible Radiation), Spectrographs, Stellar Gravitation},
     year = 1994,
    month = feb,
   volume = 107,
    pages = {742-746},
      doi = {10.1086/116893},
   adsurl = {http://adsabs.harvard.edu/abs/1994AJ....107..742G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{GrayCorbally,
	author = {{Gray}, Richard O. and {Corbally}, Christopher J.},
	title = "{Stellar Spectral Classification}",
	publisher = {Princeton University Press},
	year = 2009,
	editor = {David N. Spergel}
}

@ARTICLE{Grenier1999,
   author = {{Grenier}, S. and {Baylac}, M.-O. and {Rolland}, L. and {Burnage}, R. and 
	{Arenou}, F. and {Briot}, D. and {Delmas}, F. and {Duflot}, M. and 
	{Genty}, V. and {G{\'o}mez}, A.~E. and {Halbwachs}, J.-L. and 
	{Marouard}, M. and {Oblak}, E. and {Sellier}, A.},
    title = "{Radial velocities. Measurements of 2800 B2-F5 stars for HIPPARCOS}",
  journal = {\aaps},
 keywords = {TECHNIQUES: RADIAL VELOCITIES, STARS: EARLY-TYPE, STARS: FUNDAMENTAL PARAMETERS},
     year = 1999,
    month = jun,
   volume = 137,
    pages = {451-456},
      doi = {10.1051/aas:1999489},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999A%26AS..137..451G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Groote2004,
   author = {{Groote}, D. and {Schmitt}, J.~H.~M.~M.},
    title = "{Discovery of X-ray flaring on the magnetic Bp-star {$\sigma$} Ori E}",
  journal = {\aap},
   eprint = {astro-ph/0402437},
 keywords = {stars: chemically peculiar, stars: early-type, stars: flare, stars: individual: HD 37479, {$\sigma$} Ori E, stars: magnetic fields, stars: winds, outflows},
     year = 2004,
    month = apr,
   volume = 418,
    pages = {235-242},
      doi = {10.1051/0004-6361:20034300},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...418..235G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hannah2008,
   author = {{Hannah}, I.~G. and {Christe}, S. and {Krucker}, S. and {Hurford}, G.~J. and 
	{Hudson}, H.~S. and {Lin}, R.~P.},
    title = "{RHESSI Microflare Statistics. II. X-Ray Imaging, Spectroscopy, and Energy Distributions}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0712.2544},
 keywords = {Sun: activity, Sun: corona, Sun: flares, Sun: X-rays, gamma rays },
     year = 2008,
    month = apr,
   volume = 677,
      eid = {704-718},
    pages = {704-718},
      doi = {10.1086/529012},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677..704H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hamaguchi2000,
   author = {{Hamaguchi}, K. and {Terada}, H. and {Bamba}, A. and {Koyama}, K.
	},
    title = "{Large X-Ray Flare from the Herbig BE Star MWC 297}",
  journal = {\apj},
   eprint = {astro-ph/9911120},
 keywords = {STARS: INDIVIDUAL (MWC 297), STARS: MAGNETIC FIELDS, STARS: PRE-MAIN-SEQUENCE, X-RAYS: STARS, STARS: FLARE},
     year = 2000,
    month = apr,
   volume = 532,
    pages = {1111-1118},
      doi = {10.1086/308607},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...532.1111H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hobbs1985,
   author = {{Hobbs}, L.~M. and {Vidal-Madjar}, A. and {Ferlet}, R. and {Albert}, C.~E. and 
	{Gry}, C.},
    title = "{The gaseous component of the disk around Beta Pictoris}",
  journal = {\apjl},
 keywords = {A Stars, Gas Density, Stellar Envelopes, Stellar Spectra, Calcium, Gas Ionization, Line Spectra, Planetary Systems, Sodium},
     year = 1985,
    month = jun,
   volume = 293,
    pages = {L29-L33},
      doi = {10.1086/184485},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...293L..29H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hodgson1859,
   author = {{Hodgson}, R.},
    title = "{On a curious Appearance seen in the Sun}",
  journal = {\mnras},
     year = 1859,
    month = nov,
   volume = 20,
    pages = {15-16},
      doi = {10.1093/mnras/20.1.15},
   adsurl = {http://adsabs.harvard.edu/abs/1859MNRAS..20...15H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kallinger2010,
   author = {{Kallinger}, T. and {Matthews}, J.~M.},
    title = "{Evidence for Granulation in Early A-Type Stars}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1001.4879},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: HD50844 HD 174936, stars: oscillations, stars: variables: delta Scuti},
     year = 2010,
    month = mar,
   volume = 711,
    pages = {L35-L39},
      doi = {10.1088/2041-8205/711/1/L35},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711L..35K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kane2005,
   author = {{Kane}, S.~R. and {McTiernan}, J.~M. and {Hurley}, K.},
    title = "{Multispacecraft observations of the hard X-ray emission from the giant solar flare on 2003 November 4}",
  journal = {\aap},
 keywords = {Sun: activity, Sun: flares, Sun: X-rays, gamma rays},
     year = 2005,
    month = apr,
   volume = 433,
    pages = {1133-1138},
      doi = {10.1051/0004-6361:20041875},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...433.1133K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koch2010,
   author = {{Koch}, D.~G. and {Borucki}, W.~J. and {Basri}, G. and {Batalha}, N.~M. and 
	{Brown}, T.~M. and {Caldwell}, D. and {Christensen-Dalsgaard}, J. and 
	{Cochran}, W.~D. and {DeVore}, E. and {Dunham}, E.~W. and {Gautier}, III, T.~N. and 
	{Geary}, J.~C. and {Gilliland}, R.~L. and {Gould}, A. and {Jenkins}, J. and 
	{Kondo}, Y. and {Latham}, D.~W. and {Lissauer}, J.~J. and {Marcy}, G. and 
	{Monet}, D. and {Sasselov}, D. and {Boss}, A. and {Brownlee}, D. and 
	{Caldwell}, J. and {Dupree}, A.~K. and {Howell}, S.~B. and {Kjeldsen}, H. and 
	{Meibom}, S. and {Morrison}, D. and {Owen}, T. and {Reitsema}, H. and 
	{Tarter}, J. and {Bryson}, S.~T. and {Dotson}, J.~L. and {Gazis}, P. and 
	{Haas}, M.~R. and {Kolodziejczak}, J. and {Rowe}, J.~F. and 
	{Van Cleve}, J.~E. and {Allen}, C. and {Chandrasekaran}, H. and 
	{Clarke}, B.~D. and {Li}, J. and {Quintana}, E.~V. and {Tenenbaum}, P. and 
	{Twicken}, J.~D. and {Wu}, H.},
    title = "{Kepler Mission Design, Realized Photometric Performance, and Early Science}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1001.0268},
 primaryClass = "astro-ph.EP",
 keywords = {instrumentation: photometers, planetary systems, space vehicles: instruments, stars: statistics, stars: variables: general, techniques: photometric},
     year = 2010,
    month = apr,
   volume = 713,
      eid = {L79-L86},
    pages = {L79-L86},
      doi = {10.1088/2041-8205/713/2/L79},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713L..79K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kochukhov2007,
   author = {{Kochukhov}, O. and {Adelman}, S.~J. and {Gulliver}, A.~F. and 
	{Piskunov}, N.},
    title = "{Weather in stellar atmosphere revealed by the dynamics of mercury clouds in {$\alpha$} Andromedae}",
  journal = {Nature Physics},
archivePrefix = "arXiv",
   eprint = {0705.4469},
     year = 2007,
    month = aug,
   volume = 3,
    pages = {526-529},
      doi = {10.1038/nphys648},
   adsurl = {http://adsabs.harvard.edu/abs/2007NatPh...3..526K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Landstreet1978,
   author = {{Landstreet}, J.~D. and {Borra}, E.~F.},
    title = "{The magnetic field of Sigma Orionis E}",
  journal = {\apjl},
 keywords = {B Stars, Line Spectra, Magnetic Stars, Stellar Atmospheres, Stellar Magnetic Fields, Emission Spectra, H Alpha Line, Helium, Magnetic Equator, Variable Stars},
     year = 1978,
    month = aug,
   volume = 224,
    pages = {L5-L8},
      doi = {10.1086/182746},
   adsurl = {http://adsabs.harvard.edu/abs/1978ApJ...224L...5L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Lenz2005,
   author = {{Lenz}, P. and {Breger}, M.},
    title = "{A Magneto-Kinematic Model of the Solar Cycle}",
  journal = {CoAst},
     year = 2005,
   volume = 146,
    pages = {53}
}

@ARTICLE{Lignieres2009,
   author = {{Ligni{\`e}res}, F. and {Petit}, P. and {B{\"o}hm}, T. and {Auri{\`e}re}, M.
	},
    title = "{First evidence of a magnetic field on <ASTROBJ>Vega</ASTROBJ>. Towards a new class of magnetic A-type stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0903.1247},
 primaryClass = "astro-ph.SR",
 keywords = {stars: magnetic fields, stars: early-type, stars: individual: <ASTROBJ>Vega</ASTROBJ>},
     year = 2009,
    month = jun,
   volume = 500,
    pages = {L41-L44},
      doi = {10.1051/0004-6361/200911996},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...500L..41L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mamajek2012,
   author = {{Mamajek}, E.~E.},
    title = "{On the Age and Binarity of Fomalhaut}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1206.6353},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, circumstellar matter, planetary systems, stars: activity, stars: fundamental parameters, stars: individual: Fomalhaut TW PsA},
     year = 2012,
    month = aug,
   volume = 754,
      eid = {L20},
    pages = {L20},
      doi = {10.1088/2041-8205/754/2/L20},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754L..20M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McDonald2012,
   author = {{McDonald}, I. and {Zijlstra}, A.~A. and {Boyer}, M.~L.},
    title = "{Fundamental parameters and infrared excesses of Hipparcos stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.2037},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: fundamental parameters, Hertzsprung-Russell and colour-magnitude diagrams, stars: mass-loss, solar neighbourhood, infrared: stars},
     year = 2012,
    month = nov,
   volume = 427,
    pages = {343-357},
      doi = {10.1111/j.1365-2966.2012.21873.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.427..343M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moffat2009,
   author = {{Moffat}, A.~F.~J. and {Corcoran}, M.~F.},
    title = "{Understanding the X-ray Flaring from {$\eta$} Carinae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0910.2395},
 primaryClass = "astro-ph.HE",
 keywords = {stars: early-type, stars: individual: {$\eta$} Car LBV, X-rays: stars},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {693-704},
      doi = {10.1088/0004-637X/707/1/693},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...707..693M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morin2008,
   author = {{Morin}, J. and {Donati}, J.-F. and {Forveille}, T. and {Delfosse}, X. and 
	{Dobler}, W. and {Petit}, P. and {Jardine}, M.~M. and {Collier Cameron}, A. and 
	{Albert}, L. and {Manset}, N. and {Dintrans}, B. and {Chabrier}, G. and 
	{Valenti}, J.~A.},
    title = "{The stable magnetic field of the fully convective star V374 Peg}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0711.1418},
 keywords = {techniques: polarimetric , stars: individual: V374 Peg , stars: low-mass, brown dwarfs , stars: magnetic fields , stars: rotation},
     year = 2008,
    month = feb,
   volume = 384,
    pages = {77-86},
      doi = {10.1111/j.1365-2966.2007.12709.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.384...77M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morin2010,
   author = {{Morin}, J. and {Donati}, J.-F. and {Petit}, P. and {Delfosse}, X. and 
	{Forveille}, T. and {Jardine}, M.~M.},
    title = "{Large-scale magnetic topologies of late M dwarfs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1005.5552},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: polarimetric, stars: low-mass, stars: magnetic field, stars: rotation},
     year = 2010,
    month = oct,
   volume = 407,
    pages = {2269-2286},
      doi = {10.1111/j.1365-2966.2010.17101.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.2269M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mullan2009,
   author = {{Mullan}, D.~J.},
    title = "{Flares on a Bp Star}",
  journal = {\apj},
 keywords = {stars: early type, stars: flare, stars: magnetic fields},
     year = 2009,
    month = sep,
   volume = 702,
    pages = {759-766},
      doi = {10.1088/0004-637X/702/1/759},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702..759M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Neiner2015,
   author = {{Neiner}, C. and {Lampens}, P.},
    title = "{First discovery of a magnetic field in a main-sequence {$\delta$} Scuti star: the Kepler star HD 188774}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1508.07273},
 primaryClass = "astro-ph.SR",
 keywords = {stars: individual: HD 188774, stars: magnetic field, stars: oscillations, starspots, stars: variables: {$\delta$} Scuti},
     year = 2015,
    month = nov,
   volume = 454,
    pages = {L86-L90},
      doi = {10.1093/mnrasl/slv130},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.454L..86N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Owocki2007,
   author = {{Owocki}, S. and {Townsend}, R. and {Ud-Doula}, A.},
    title = "{Modeling the magnetospheres of luminous stars: Interactions between supersonic radiation-driven winds and stellar magnetic fields}",
  journal = {Physics of Plasmas},
 keywords = {Stellar atmospheres, radiative transfer, opacity and line formation, Luminosities, magnitudes, effective temperatures colors and spectral classification, Magnetic and electric fields, polarization of starlight, Mass loss and stellar winds, Main-sequence: early-type stars, Hydrodynamics},
     year = 2007,
    month = may,
   volume = 14,
   number = 5,
    pages = {056502-056502},
      doi = {10.1063/1.2472340},
   adsurl = {http://adsabs.harvard.edu/abs/2007PhPl...14e6502O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petit2011,
   author = {{Petit}, P. and {Ligni{\`e}res}, F. and {Auri{\`e}re}, M. and 
	{Wade}, G.~A. and {Alina}, D. and {Ballot}, J. and {B{\"o}hm}, T. and 
	{Jouve}, L. and {Oza}, A. and {Paletou}, F. and {Th{\'e}ado}, S.
	},
    title = "{Detection of a weak surface magnetic field on Sirius A: are all tepid stars magnetic?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1106.5363},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, stars: magnetic field, stars: rotation, stars: individual: Sirius A},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {L13},
    pages = {L13},
      doi = {10.1051/0004-6361/201117573},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532L..13P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petit2015,
   author = {{Petit}, V. and {Cohen}, D.~H. and {Wade}, G.~A. and {Naz{\'e}}, Y. and 
	{Owocki}, S.~P. and {Sundqvist}, J.~O. and {ud-Doula}, A. and 
	{Fullerton}, A. and {Leutenegger}, M. and {Gagn{\'e}}, M.},
    title = "{X-ray emission from the giant magnetosphere of the magnetic O-type star NGC 1624-2}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1507.08621},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: individual: NGC 1624-2, stars: magnetic field, stars: massive, stars: winds, outflows, X-rays: stars},
     year = 2015,
    month = nov,
   volume = 453,
    pages = {3288-3299},
      doi = {10.1093/mnras/stv1741},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.453.3288P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pittard2002,
   author = {{Pittard}, J.~M. and {Corcoran}, M.~F.},
    title = "{In hot pursuit of the hidden companion of eta Carinae: An X-ray determination of the wind parameters}",
  journal = {\aap},
   eprint = {astro-ph/0201105},
 keywords = {STARS: BINARIES: GENERAL, STARS: EARLY-TYPE, STARS: INDIVIDUAL: ETA CARINAE, STARS: WOLF-RAYET, X-RAYS: STARS},
     year = 2002,
    month = feb,
   volume = 383,
    pages = {636-647},
      doi = {10.1051/0004-6361:20020025},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...383..636P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Power2007,
   author = {{Power}, J. and {Wade}, G.~A. and {Hanes}, D.~A. and {Aurier}, M. and 
	{Silvester}, J.},
    title = "{Properties of a volume-limited sample of magnetic Ap/Bp stars}",
booktitle = {Physics of Magnetic Stars},
     year = 2007,
   eprint = {astro-ph/0612557},
   editor = {{Romanyuk}, I.~I. and {Kudryavtsev}, D.~O. and {Neizvestnaya}, O.~M. and 
	{Shapoval}, V.~M.},
    pages = {89-97},
   adsurl = {http://adsabs.harvard.edu/abs/2007pms..conf...89P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Robrade2011,
   author = {{Robrade}, J. and {Schmitt}, J.~H.~M.~M.},
    title = "{New X-ray observations of IQ Aurigae and {$\alpha$}$^{2}$ Canum Venaticorum. Probing the magnetically channeled wind shock model in A0p stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1105.3688},
 primaryClass = "astro-ph.SR",
 keywords = {stars: activity, stars: chemically peculiar, stars: individual:{$\alpha$}2CVn, stars: individual: IQ Aur, X-rays: stars},
     year = 2011,
    month = jul,
   volume = 531,
      eid = {A58},
    pages = {A58},
      doi = {10.1051/0004-6361/201116843},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...531A..58R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Rosner1980,
   author = {{Rosner}, R. and {Vaiana}, G.~S.},
    title = "{Stellar coronae from Einstein - Observations and theory}",
 keywords = {Stellar Coronas, Stellar Evolution, X Ray Astronomy, X Ray Sources, Early Stars, Giant Stars, Late Stars, Solar Corona, Spaceborne Astronomy, Stellar Magnetic Fields, Supergiant Stars},
booktitle = {NATO Advanced Science Institutes (ASI) Series C},
     year = 1980,
   series = {NATO Advanced Science Institutes (ASI) Series C},
   volume = 60,
   editor = {{Giacconi}, R. and {Setti}, G.},
    pages = {129-151},
   adsurl = {http://adsabs.harvard.edu/abs/1980ASIC...60..129R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanchez2013,
   author = {{Sanchez}, S. and {Fournier}, A. and {Pinheiro}, K. and {Aubert}, J.
	},
    title = "{A mean-field Babcock-Leighton solar dynamo model with long-term variability}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1307.4115},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2013,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1307.4115S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sanz-Forcada2004,
   author = {{Sanz-Forcada}, J. and {Franciosini}, E. and {Pallavicini}, R.
	},
    title = "{XMM-Newton observations of the {$\sigma$} Ori cluster. I. The complex RGS spectrum of the hot star {$\sigma$} Ori AB}",
  journal = {\aap},
   eprint = {astro-ph/0404078},
 keywords = {stars: coronae, stars: winds, outflows, stars: individual: {$\sigma$} Ori, stars: early-type, stars: late-type},
     year = 2004,
    month = jul,
   volume = 421,
    pages = {715-727},
      doi = {10.1051/0004-6361:20047159},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421..715S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schmitt2004,
   author = {{Schmitt}, J.~H.~M.~M. and {Liefke}, C.},
    title = "{NEXXUS: A comprehensive ROSAT survey of coronal X-ray emission among nearby solar-like stars}",
  journal = {\aap},
   eprint = {astro-ph/0308510},
 keywords = {stars: activity, stars: coronae, stars: late-type, X-rays: stars},
     year = 2004,
    month = apr,
   volume = 417,
    pages = {651-665},
      doi = {10.1051/0004-6361:20030495},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...417..651S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shibata2011,
   author = {{Shibata}, K. and {Magara}, T.},
    title = "{Solar Flares: Magnetohydrodynamic Processes}",
  journal = {Living Rev. Solar Phys.},
     year = 2011,
   volume = 8,
    pages = {6},
   adsurl = {http://www.livingreviews.org/lrsp-2011-6}
}


@ARTICLE{Shibayama2013,
   author = {{Shibayama}, T. and {Maehara}, H. and {Notsu}, S. and {Notsu}, Y. and 
	{Nagao}, T. and {Honda}, S. and {Ishii}, T.~T. and {Nogami}, D. and 
	{Shibata}, K.},
    title = "{Superflares on Solar-type Stars Observed with Kepler. I. Statistical Properties of Superflares}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1308.1480},
 primaryClass = "astro-ph.SR",
 keywords = {stars: activity, stars: flare, stars: rotation, stars: solar-type, starspots},
     year = 2013,
    month = nov,
   volume = 209,
      eid = {5},
    pages = {5},
      doi = {10.1088/0067-0049/209/1/5},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..209....5S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Slettebak1975,
   author = {{Slettebak}, A.},
    title = "{Some interesting bright southern stars of early type.}",
  journal = {\apj},
     year = 1975,
    month = apr,
   volume = 197,
    pages = {137-138},
      doi = {10.1086/153493},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...197..137S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Slettebak1982,
   author = {{Slettebak}, A.},
    title = "{Spectral types and rotational velocities of the brighter Be stars and A-F type shell stars}",
  journal = {\apjs},
 keywords = {B Stars, F Stars, Shell Stars, Stellar Envelopes, Stellar Rotation, Stellar Spectra, A Stars, Angular Velocity, Astronomical Catalogs, Stellar Luminosity, Tables (Data)},
     year = 1982,
    month = sep,
   volume = 50,
    pages = {55-83},
      doi = {10.1086/190820},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJS...50...55S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Smith1993,
   author = {{Smith}, M.~A. and {Grady}, C.~A. and {Peters}, G.~J. and {Feigelson}, E.~D.
	},
    title = "{A giant X-ray flare on Lambda Eridani (B2e)}",
  journal = {\apjl},
 keywords = {B Stars, Rosat Mission, Stellar Flares, Stellar Luminosity, Stellar Radiation, Iue, Proportional Counters, X Rays},
     year = 1993,
    month = jun,
   volume = 409,
    pages = {L49-L52},
      doi = {10.1086/186857},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...409L..49S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Steck2008,
   author = {{Steck}, D.~A.},
    title = "{Sodium D Line Data}",
  howpublished = {available online at \url{http://steck.us/alkalidata}},
     year = 2008,
   volume = {revision 2.0.1}
}


@ARTICLE{Stelzer2005,
   author = {{Stelzer}, B. and {Flaccomio}, E. and {Montmerle}, T. and {Micela}, G. and 
	{Sciortino}, S. and {Favata}, F. and {Preibisch}, T. and {Feigelson}, E.~D.
	},
    title = "{X-Ray Emission from Early-Type Stars in the Orion Nebula Cluster}",
  journal = {\apjs},
   eprint = {astro-ph/0505503},
 keywords = {Stars: Binaries: General, Galaxy: Open Clusters and Associations: Individual: Name: Orion Nebula Cluster, Stars: Early-Type, Stars: Pre-Main-Sequence, Stars: Winds, Outflows, X-Rays: Stars},
     year = 2005,
    month = oct,
   volume = 160,
    pages = {557-581},
      doi = {10.1086/432375},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJS..160..557S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skrutskie2006,
   author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and 
	{Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and 
	{Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and 
	{Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and 
	{Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and 
	{Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and 
	{Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and 
	{Wheelock}, S.},
    title = "{The Two Micron All Sky Survey (2MASS)}",
  journal = {\aj},
 keywords = {Catalogs, Infrared: General, Surveys},
     year = 2006,
    month = feb,
   volume = 131,
    pages = {1163-1183},
      doi = {10.1086/498708},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1163S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Spitzer1978,
	author = {{Spitzer}, L.},
	title = "{Physical processes in the interstellar medium}",
	publisher = {New York: John Wiley \& Sons},
	year = 1978
}

@ARTICLE{Telting2014,
   author = {{Telting}, J.~H. and {Avila}, G. and {Buchhave}, L. and {Frandsen}, S. and 
	{Gandolfi}, D. and {Lindberg}, B. and {Stempels}, H.~C. and 
	{Prins}, S. and {NOT staff}},
    title = "{FIES: The high-resolution Fiber-fed Echelle Spectrograph at the Nordic Optical Telescope}",
  journal = {Astronomische Nachrichten},
 keywords = {instrumentation: spectrographs, techniques: radial velocities, techniques: spectroscopic},
     year = 2014,
    month = jan,
   volume = 335,
    pages = {41},
      doi = {10.1002/asna.201312007},
   adsurl = {http://adsabs.harvard.edu/abs/2014AN....335...41T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thompson2012,
   author = {{Thompson}, S.~E. and {Everett}, M. and {Mullally}, F. and {Barclay}, T. and 
	{Howell}, S.~B. and {Still}, M. and {Rowe}, J. and {Christiansen}, J.~L. and 
	{Kurtz}, D.~W. and {Hambleton}, K. and {Twicken}, J.~D. and 
	{Ibrahim}, K.~A. and {Clarke}, B.~D.},
    title = "{A Class of Eccentric Binaries with Dynamic Tidal Distortions Discovered with Kepler}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1203.6115},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: general, stars: evolution, stars: oscillations: including pulsations, stars: variables: general},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {86},
    pages = {86},
      doi = {10.1088/0004-637X/753/1/86},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753...86T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tkachenko2013,
   author = {{Tkachenko}, A. and {Lehmann}, H. and {Smalley}, B. and {Uytterhoeven}, K.
	},
    title = "{Spectrum analysis of bright Kepler late B- to early F-stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1303.2934},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: fundamental parameters, stars: variables: {$\delta$} Scuti},
     year = 2013,
    month = jun,
   volume = 431,
    pages = {3685-3696},
      doi = {10.1093/mnras/stt453},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.431.3685T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Tody1986,
   author = {{Tody}, D.},
    title = "{The IRAF Data Reduction and Analysis System}",
booktitle = {Instrumentation in astronomy VI},
     year = 1986,
   series = {\procspie},
   volume = 627,
   editor = {{Crawford}, D.~L.},
    month = jan,
    pages = {733},
   adsurl = {http://adsabs.harvard.edu/abs/1986SPIE..627..733T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Tody1993,
   author = {{Tody}, D.},
    title = "{IRAF in the Nineties}",
booktitle = {Astronomical Data Analysis Software and Systems II},
     year = 1993,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 52,
   editor = {{Hanisch}, R.~J. and {Brissenden}, R.~J.~V. and {Barnes}, J.
	},
    month = jan,
    pages = {173},
   adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...52..173T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Townsend2005,
   author = {{Townsend}, R.~H.~D. and {Owocki}, S.~P.},
    title = "{A rigidly rotating magnetosphere model for circumstellar emission from magnetic OB stars}",
  journal = {\mnras},
   eprint = {astro-ph/0408565},
 keywords = {stars: chemically peculiar, stars: early-type, stars: emission-line, Be, stars: magnetic fields, stars: mass-loss, stars: rotation},
     year = 2005,
    month = feb,
   volume = 357,
    pages = {251-264},
      doi = {10.1111/j.1365-2966.2005.08642.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.357..251T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Vallerga1993,
   author = {{Vallerga}, J.~V. and {Vedder}, P.~W. and {Craig}, N. and {Welsh}, B.~Y.
	},
    title = "{High-resolution CA II observations of the local interstellar medium}",
  journal = {\apj},
 keywords = {Calcium, Clouds, Early Stars, Interstellar Gas, Interstellar Matter, Metal Ions, High Resolution, Ion Charge, Line Of Sight, Line Spectra},
     year = 1993,
    month = jul,
   volume = 411,
    pages = {729-749},
      doi = {10.1086/172875},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...411..729V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{VanCleve2009,
   author = {{Van Cleve}, J. and {Caldwell}, D. and {Thompson}, R. and {Haas}, M.~R. and {Koch}, D. and {Borucki}, W.~J.},
    title = "{Kepler Instrument Handbook, KSCI 19033-001}",
booktitle = {Kepler Instrument Handbook},
     year = 2009,
   adsurl = {http://archive.stsci.edu/kepler/manuals/KSCI-19033-001.pdf},
  Publisher = {NASA Ames Research Center}
}

@ARTICLE{Verner2005,
   author = {{Verner}, E. and {Bruhweiler}, F. and {Gull}, T.},
    title = "{The Binarity of {$\eta$} Carinae Revealed from Photoionization Modeling of the Spectral Variability of the Weigelt Blobs B and D}",
  journal = {\apj},
   eprint = {astro-ph/0502106},
 keywords = {Atomic Data, ISM: H II Regions, ISM: Individual: Name: {$\eta$} Carinae, Line: Formation, Line: Identification},
     year = 2005,
    month = may,
   volume = 624,
    pages = {973-982},
      doi = {10.1086/429400},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...624..973V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vink2005,
   author = {{Vink}, J.~S. and {O'Neill}, P.~M. and {Els}, S.~G. and {Drew}, J.~E.
	},
    title = "{On the origin of the X-ray emission towards the early Herbig Be star MWC 297}",
  journal = {\aap},
   eprint = {astro-ph/0506271},
 keywords = {stars: formation, stars: pre-main sequence, stars: flare, stars: individual: M 297, X-rays: stars},
     year = 2005,
    month = aug,
   volume = 438,
    pages = {L21-L24},
      doi = {10.1051/0004-6361:200500141},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005A%26A...438L..21V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walkowicz2011,
   author = {{Walkowicz}, L.~M. and {Basri}, G. and {Batalha}, N. and {Gilliland}, R.~L. and 
	{Jenkins}, J. and {Borucki}, W.~J. and {Koch}, D. and {Caldwell}, D. and 
	{Dupree}, A.~K. and {Latham}, D.~W. and {Meibom}, S. and {Howell}, S. and 
	{Brown}, T.~M. and {Bryson}, S.},
    title = "{White-light Flares on Cool Stars in the Kepler Quarter 1 Data}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1008.0853},
 primaryClass = "astro-ph.SR",
 keywords = {stars: emission-line, Be, stars: flare, stars: low-mass},
     year = 2011,
    month = feb,
   volume = 141,
      eid = {50},
    pages = {50},
      doi = {10.1088/0004-6256/141/2/50},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....141...50W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Welsh2010,
   author = {{Welsh}, B.~Y. and {Lallement}, R. and {Vergely}, J.-L. and 
	{Raimond}, S.},
    title = "{New 3D gas density maps of NaI and CaII interstellar absorption within 300 pc}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0912.3040},
 keywords = {solar neighborhood, ISM: atoms, ISM: clouds},
     year = 2010,
    month = feb,
   volume = 510,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/200913202},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...510A..54W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Welsh2011,
   author = {{Welsh}, W.~F. and {Orosz}, J.~A. and {Aerts}, C. and {Brown}, T.~M. and 
	{Brugamyer}, E. and {Cochran}, W.~D. and {Gilliland}, R.~L. and 
	{Guzik}, J.~A. and {Kurtz}, D.~W. and {Latham}, D.~W. and {Marcy}, G.~W. and 
	{Quinn}, S.~N. and {Zima}, W. and {Allen}, C. and {Batalha}, N.~M. and 
	{Bryson}, S. and {Buchhave}, L.~A. and {Caldwell}, D.~A. and 
	{Gautier}, III, T.~N. and {Howell}, S.~B. and {Kinemuchi}, K. and 
	{Ibrahim}, K.~A. and {Isaacson}, H. and {Jenkins}, J.~M. and 
	{Prsa}, A. and {Still}, M. and {Street}, R. and {Wohler}, B. and 
	{Koch}, D.~G. and {Borucki}, W.~J.},
    title = "{KOI-54: The Kepler Discovery of Tidally Excited Pulsations and Brightenings in a Highly Eccentric Binary}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1102.1730},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: close, binaries: spectroscopic, stars: individual: KID 8112039 HD 187091 2MASS J19461553+4356513, stars: oscillations, stars: variables: general},
     year = 2011,
    month = nov,
   volume = 197,
      eid = {4},
    pages = {4},
      doi = {10.1088/0067-0049/197/1/4},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..197....4W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

